Active Sybil attack and efficient defense strategy in IPFS DHT

The InterPlanetary File System (IPFS) is a decentralized peer-to-peer (P2P) storage built on Kademlia, a Distributed Hash Table (DHT) structure commonly used in P2P systems and known for its proved scalability. However, DHTs susceptible to Sybil attacks, where a single entity controls multiple malicious nodes. Recent studies have shown that IPFS is affected by a passive content eclipse attack, leveraging Sybils, in which adversarial nodes hide received indexed information from other peers, making the content appear unavailable. Fortunately, the latest mitigation strategy coupling an attack detection based on statistical tests and a wider publication strategy upon detection was able to circumvent it. In this work, we present a new active attack in which malicious nodes return semantically correct but intentionally false data. The attack leverages strategic Sybil placement to evade detection and exploits an early termination in the actual Kubo, the main IPFS implementation. It achieves to fully eclipse content on recent Kubo versions. When evaluated against the most recent known mitigation, it successfully denies access to the target content in approximately 80% of lookup attempts. To address this vulnerability, we propose a new mitigation called SR-DHT-Store, which enables efficient, Sybil-resistant content publication without relying on attack detection. Instead, it uses systematic and precise use of region-based queries based on a dynamically computed XOR distance to the target ID. SR-DHT-Store can be combined with other defense mechanisms, fully mitigating passive and active Sybil attacks at a lower overhead while supporting an incremental deployment.

==> src/header.tex <==
\RequirePackage[OT1]{fontenc}

%%%%%%%%%%%%%%
%% Packages %%
% List of all packages imported
\usepackage{times}
\usepackage{mathptmx} 
\usepackage{cite} % Hyperlinks
\usepackage{amsmath,amssymb,amsfonts} % Special math characters
\usepackage{graphicx} % Images
\usepackage{textcomp}
\usepackage[table,xcdraw,dvipsnames]{xcolor} % Add colors to text
% \usepackage[htt]{hyphenat}
\usepackage{microtype} % Allow work breaks in texttt
\usepackage{algpseudocode}
\usepackage{algorithm}
\usepackage{tabularray, makecell} % Tabularray tables
\renewcommand\ttdefault{cmvtt}
\usepackage[labelsep=colon]{caption}
% \usepackage[switch]{lineno} % Add line number
% \linenumbers

% \usepackage{lmodern}%ajout thibault pour compiler

% For citation
\newcommand{\citep}[1]{\cite{#1}}
\newcommand{\citet}[2]{#1~\cite{#2}}

\usepackage{listings} % Add lstlisting for code blocks
\lstset{ % "listings" package configuration
    frame=single,
    basicstyle=\footnotesize,
    keywordstyle=\color{red},
    numbers=left,
    numbersep=-5pt,
    showstringspaces=false, 
    stringstyle=\color{blue},
    tabsize=4,
    captionpos=b
}

\usepackage{xurl}
\usepackage[colorlinks = true, urlcolor  = blue, citecolor = blue]{hyperref}

% \corref hyperref error when handling the corresponding author (*).
\pdfstringdefDisableCommands{%
  \def\corref#1{*}%
}
%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%
%% Commands %%
% List of commands used
\newcommand{\todo}[1]{\textcolor{red}{TODO: #1}}
\newcommand{\tc}[1]{\textcolor{Violet}{TC: #1}}
\newcommand{\ci}[1]{\textcolor{Magenta}{CI: #1}}
\newcommand{\vdmn}[1]{\textcolor{Turquoise}{VDMN: #1}}
\colorlet{Review}{ForestGreen!200}
% \definecolor{Review}{HTML}{0f8c5f}
\newenvironment{review}
  {\color{Review}}
  {}
\setlength{\fboxrule}{0.5mm} % Thickness of borders in figures for review


% For the et al.
\newcommand{\etal}{\textit{et al. }}
%%%%%%%%%%%%%%

